AdaAfford: Learning to Adapt Manipulation Affordance for 3D Articulated Objects via Few-shot Interactions

Perceiving and interacting with 3D articulated objects, such as cabinets, doors, and faucets, pose particular challenges for future home-assistant robots performing daily tasks in human environments. Besides parsing the articulated parts and joint parameters, researchers recently advocate learning manipulation affordance over the input shape geometry which is more task-aware and geometrically fine-grained. However, taking only passive observations as inputs, these methods ignore many hidden but important kinematic constraints (e.g., joint location and limits) and dynamic factors (e.g., joint friction and restitution), therefore losing significant accuracy for test cases with such uncertainties. In this paper, we propose a novel framework, named AdaAfford, that learns to perform very few test-time interactions for quickly adapting the affordance priors to more accurate instance-specific posteriors. We conduct large-scale experiments using the PartNet-Mobility dataset and prove that our system performs better than baselines.

==> tabs/fulltable.tex <==
\begin{table*}[t]
  \centering
    \setlength{\tabcolsep}{5pt}
  \renewcommand\arraystretch{0.5}
  \small
\begin{tabular}{@{}llcccccc@{}}
\toprule
& &  F-score (\%) & Precision (\%) & Recall (\%) & Avg-Acc (\%) & Sample-Succ (\%)\\
\midrule
\multirow{7}{*}{pushing all categories}
& Where2Act &  56.44 / {49.95} & 48.25 / {56.90} & 67.99 / {44.52} & 63.16 / {56.41} & 20.85 / {21.69}\\
& ours-random 1 interactions&  69.09/57.71 & 79.21/61.44 & 61.27/54.40 & 72.60/61.04 & 29.86/29.09\\
& ours-random 2 interactions&  69.45/55.35 & 80.78/62.24 & 60.90/49.83 & 73.21/60.71 & 28.65/31.04\\
& ours-random 4 interactions&  40.18/53.47 & 77.25/64.96 & 27.15/45.43 & 59.58/61.36 & 25.27/32.08\\
& ours-AIP 1 interaction &  {70.50} / {58.44} & {63.13} / {59.45} & \textbf{79.81} / \textbf{57.48} & {76.12} / {60.06} & \textbf{35.70} / {30.00}\\
& ours-AIP 2 interactions &  {73.96} / {58.06} & {70.77} / {61.10} & {77.45} / 55.32 & \textbf{80.50} / {60.96} & {35.50} / {30.39}\\
& ours-AIP 4 interactions &  \textbf{74.63} / \textbf{60.38} & \textbf{74.98} / {74.76} & {74.30} / {50.64} & {74.74} / \textbf{67.81} & {35.14} / \textbf{33.50}\\
\midrule
\multirow{7}{*}{pulling all categories}
& Where2Act &  {31.19} / 36.36 & {22.22} / \textbf{63.16} & \textbf{52.30} / 25.53 & {57.38} / 57.19 & 1.92 / {10.00}\\
& ours-random 1 interactions&  28.58/15.09 & 33.10/26.23 & 25.16/10.60 & 63.72/68.75 & 3.89/8.70\\
& ours-random 2 interactions&  24.40/44.32 & 35.72/53.50 & 18.54/37.84 & 67.71/71.33 & 3.33/4.78\\
& ours-random 4 interactions&  15.09/38.24 & 26.23/62.89 & 10.60/27.48 & 68.75/\textbf{73.23} & 3.89/10.00\\
& ours-AIP 1 interaction &  {35.73} / {39.10} & {31.63} / {44.07} & {41.05} / 35.14 & {61.28} / {66.98} & {3.33} / {10.45}\\
& ours-AIP 2 interactions &  {37.20} / {35.29} & {34.46} / {56.44} & {40.40} / 25.68 & {64.24} / {71.60} & {6.67} / {10.83}\\
& ours-AIP 4 interactions &  \textbf{37.50} / \textbf{49.78} & \textbf{42.15} / {48.71} & {33.77} / \textbf{50.90} & \textbf{70.49} / {69.02} & \textbf{9.44} / \textbf{10.87}\\
\midrule
\multirow{9}{*}{pulling closed door}
& Where2Act & 48.44 & 44.20 & 53.58 & 59.28 & 4.38\\
& ours-random 1 interactions&  61.41 & 58.76 & 64.31 & 77.77 & 7.73\\
& ours-random 2 interactions&  57.67 & 56.22 & 59.19 & 75.62 & 9.125\\
& ours-random 4 interactions&  64.96 & 63.24 & 66.78 & 79.87 & 9.56\\
& ours-AIP 1 interaction &  {56.11} & {53.30} & {59.23} & {75.19} & {7.63}\\
& ours-AIP 2 interactions &  {58.68} & {54.77} & {63.19} & {75.53} & {11.36}\\
& ours-AIP 4 interactions &  \textbf{67.68} & \textbf{66.46}  & \textbf{68.94} & \textbf{81.59} & \textbf{17.08}\\
\midrule
\multirow{9}{*}{pushing faucet}
& Where2Act &  20.08 & 29.31 & 15.28 & 59.75 & 26.59\\
& ours-random 1 interactions&  76.60 & \textbf{82.20} & 71.71 & 84.72 & 35.46\\
& ours-random 2 interactions&  76.08 & 79.93 & 72.58 & 84.17 & 35.57\\
& ours-random 4 interactions&  77.98 & 79.85 & 76.20 & 85.31 & 39.25\\
& ours-AIP 1 interaction &  76.01 & 81.45 & 71.25 & 84.40 & 36.53\\
& ours-AIP 2 interactions &  76.93 & 78.81 & 75.13 & 84.74 & 46.23\\
& ours-AIP 4 interactions & \textbf{78.40} & 79.94 & \textbf{76.92} & \textbf{85.57} & \textbf{50.44}

\\
\bottomrule
\end{tabular}
  \caption{\textbf{Quantitative Evaluations and Comparisons.} We compare our method to two baseline methods: the Where2Act~\cite{Mo_2021_ICCV} approach that ignores the hidden information and the ours-random baseline that replaces the interaction candidates proposed by our \textit{Adaptive Interaction Proposal} module with random ones.
  We set three different test-time interaction budgets where only 1, 2, or 4 interactions are allowed.
  For all metrics, higher numbers indicate better performance.
  For the experiments over all categories, we report the performance over novel shapes from the training categories and shapes from novel categories before and after the slash.
  }
  \vspace{-3mm}
  \label{tab:numbers}
\end{table*}%%

==> tabs/supp_table.tex <==
\begin{table}[t]
  \centering
    \setlength{\tabcolsep}{3pt}
  \renewcommand\arraystretch{0.5}
  \footnotesize
\begin{tabular}{@{}llccc@{}}
\toprule
 &  &  F-score (\%) & Sample-Succ (\%)\\
\midrule
% \multirow{2}{*}{\shortstack[l]{pushing all (train cat.)}}
pushing all
& ours-w/o attention &  69.61/68.84/69.49 & 32.84/35.00/34.05 \\
% & ours-heuristic &  69.09 / 69.45 / 72.28 & 29.86 / 28.65 / 25.27 \\
(train cat.) & ours-final &  \textbf{70.50} / \textbf{73.96} / \textbf{74.63} & \textbf{35.70} / \textbf{35.50} / \textbf{35.14} \\
\midrule
% \multirow{2}{*}{\shortstack[l]{pushing all\\(test cat.)}}
pushing all
& ours-w/o attention &  49.26/52.31/53.60 & 27.53/\textbf{32.08}/31.94 \\
% & ours-heuristic &  57.71 / 55.35 / 53.47 & 29.09 / \textbf{31.04} / 32.08 \\
(test cat.)
& ours-final &  \textbf{58.44} / \textbf{58.06} / \textbf{60.38} & \textbf{30.00} / 30.39 / \textbf{33.50} \\
\midrule
% \multirow{2}{*}{\shortstack[l]{pulling all\\(train cat.)}}
pulling all
& ours-w/o attention & \textbf{35.84}/34.77/34.63  & 1.88/2.81/4.96 \\
% & ours-heuristic & 28.58 / 24.40 / 15.09  & \textbf{3.89} / 3.33 / 3.89 \\
(train cat.)
& ours-final & 35.73 / \textbf{37.20} / \textbf{37.50}  & \textbf{3.33} / \textbf{6.67} / \textbf{9.44} \\
\midrule
% \multirow{2}{*}{\shortstack[l]{pulling all\\(test cat.)}}
pulling all
& ours-w/o attention & 38.25/\textbf{39.01}/39.58  & 4.70/2.94/2.65 \\%  7.39/6.96/9.13
% & ours-heuristic & 15.09 / \textbf{44.32} / 38.24  &  8.70 / 4.78 / 10.00\\
(test cat.)
& ours-final &  \textbf{39.10} / 35.29 / \textbf{49.78} & \textbf{10.45} / \textbf{10.83} / \textbf{10.87} \\
\midrule
% \multirow{2}{*}{\shortstack[l]{pulling\\closed door}}
pulling
& ours-w/o attention & 49.69/51.40/50.24 & \textbf{9.66}/8.49/15.58\\
% & ours-heuristic &  51.37 / 57.67 / 64.96 & 7.41 / 9.13 / 9.56\\
closed door
& ours-final  &  \textbf{56.11} / \textbf{58.68} / \textbf{67.68} & 7.63 / \textbf{11.36} / \textbf{17.08} \\
\midrule
% \multirow{2}{*}{\shortstack[l]{pushing\\faucet}}
pushing
& ours-w/o attention &  72.59/72.52/69.03 & 32.61/31.71/37.81\\
% & ours-heuristic &  \textbf{76.60} / 76.08 / 77.98 & 35.46 / 35.57 / 39.25\\
faucet
& ours-final  &  \textbf{76.01} / \textbf{76.93} / \textbf{78.40} & \textbf{36.53} / \textbf{46.23} / \textbf{50.44} \\
\bottomrule
\end{tabular}
  \caption{\textbf{Quantitative Evaluations and Comparisons.} We compare our method with the "ours-w/o attention" approach that removes the attention score in Adaptive Information Encoder.
  We experiment with three different test-time interaction budgets (\ie, 1, 2, or 4) and report the numbers separated by slashes.
  We use "pushing all" and "pulling all" to denote the experiments over all object categories, while "puling closed door" and "pushing faucet" refer to the experiments over a single category only.
  For the experiments over all categories, we report the performance over novel shapes from the training categories (marked with "train cat.") and shapes from novel categories (marked with "test cat.").
  We see clearly that ours-final achieves the best performance in most comparison entries.
  }
  \vspace{-3mm}
  \label{tab:supp_numbers}
\end{table}%%

==> tabs/tmptable.tex <==
\begin{table}[t]
  \centering
    \setlength{\tabcolsep}{5pt}
  \renewcommand\arraystretch{0.5}
  \footnotesize
\begin{tabular}{@{}llccc@{}}
\toprule
& &  F-score (\%) & Sample-Succ (\%)\\
\midrule
\multirow{3}{*}{\shortstack[l]{pushing all\\(train cat.)}}
& Where2Act &  56.44 & 20.85 \\
& ours-random &  69.09 / 69.45 / 40.18 & 29.86 / 28.65 / 25.27 \\
& ours-AIP &  {70.50} / {73.96} / \textbf{74.63} & \textbf{35.70} / {35.50} / {35.14} \\
\midrule
\end{tabular}
  \caption{\textbf{Quantitative Evaluations and Comparisons.} We compare our method to two baseline methods: the Where2Act~\cite{Mo_2021_ICCV} approach that ignores the hidden information and the ours-random baseline that replaces the interaction candidates proposed by our \textit{Adaptive Interaction Proposal} module with random ones.
  We set three different test-time interaction budgets where only 1, 2, or 4 interactions are allowed.
  For all metrics, higher numbers indicate better performance.
  For the experiments over all categories, we report the performance over novel shapes from the training categories and shapes from novel categories before and after the slash.
  }
  \vspace{-3mm}
  \label{tab:numbers}
\end{table}%%

==> tex/supp_failure.tex <==
\section{Failure Cases and Analysis}



\begin{figure}[t]
    \begin{center}
        \includegraphics[width=\linewidth, 
        trim={0cm, 0cm, 0cm, 0cm}, clip]{figures/none.png}
    \end{center}
    \caption{\textbf{Failure Cases.}
    }
    \label{fig:failure}
\end{figure}
